Centroid adapted frequency selective extrapolation for reconstruction of lost image areas

Lost image areas with different size and arbitrary shape can occur in many scenarios such as error-prone communication, depth-based image rendering or motion compensated wavelet lifting. The goal of image reconstruction is to restore these lost image areas as close to the original as possible. Frequency selective extrapolation is a block-based method for efficiently reconstructing lost areas in images. So far, the actual shape of the lost area is not considered directly. We propose a centroid adaption to enhance the existing frequency selective extrapolation algorithm that takes the shape of lost areas into account. To enlarge the test set for evaluation we further propose a method to generate arbitrarily shaped lost areas. On our large test set, we obtain an average reconstruction gain of 1.29 dB.

==> border_tab/psnr-tab-arri.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 32.605 & 32.621 & 31.945 & 32.124 & 30.694 & 31.313\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.016 } & \multicolumn{2}{c}{ + 0.179 } & \multicolumn{2}{c}{ + 0.619 }\tabularnewline


==> border_tab/psnr-tab-arri_ref.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 27.580 & 26.832 & 28.762 & 29.466 & 32.605 & 32.621 & 31.945 & 32.124 & 30.694 & 31.313\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.016 } & \multicolumn{2}{c}{ + 0.179 } & \multicolumn{2}{c}{ + 0.619 }\tabularnewline


==> border_tab/psnr-tab-kodak.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 25.718 & 25.725 & 25.355 & 25.470 & 24.607 & 24.965\tabularnewline
 & & \multicolumn{2}{c}{ + 0.007 } & \multicolumn{2}{c}{ + 0.115 } & \multicolumn{2}{c}{ + 0.358 }\tabularnewline


==> border_tab/psnr-tab-kodak_ref.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 22.310 & 21.835 & 23.780 & 23.897 & 25.718 & 25.725 & 25.355 & 25.470 & 24.607 & 24.965\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.007 } & \multicolumn{2}{c}{ + 0.115 } & \multicolumn{2}{c}{ + 0.358 }\tabularnewline


==> border_tab/psnr-tab-middleburry.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 35.086 & 35.094 & 34.388 & 34.551 & 33.355 & 33.943\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.008 } & \multicolumn{2}{c}{ + 0.163 } & \multicolumn{2}{c}{ + 0.588 }\tabularnewline


==> border_tab/psnr-tab-middleburry_ref.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 29.032 & 27.997 & 31.428 & 31.791 & 35.086 & 35.094 & 34.388 & 34.551 & 33.355 & 33.943\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.008 } & \multicolumn{2}{c}{ + 0.163 } & \multicolumn{2}{c}{ + 0.588 }\tabularnewline


==> border_tab/psnr-tab-tecnick.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 28.129 & 28.138 & 27.557 & 27.704 & 26.680 & 27.186\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.009 } & \multicolumn{2}{c}{ + 0.147 } & \multicolumn{2}{c}{ + 0.506 }\tabularnewline


==> border_tab/psnr-tab-tecnick_ref.tex <==
& \multirow{2}{*}{\textit{Tecnick}}  & 23.954 & 23.378 & 25.364 & 25.601 & 28.129 & 28.138 & 27.557 & 27.704 & 26.680 & 27.186\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.009 } & \multicolumn{2}{c}{ + 0.147 } & \multicolumn{2}{c}{ + 0.506 }\tabularnewline


==> border_tab/psnr_err2-tab-arri.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 37.776 & 37.845 & 36.980 & 37.569 & 34.697 & 36.552\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.069 } & \multicolumn{2}{c}{ + 0.589 } & \multicolumn{2}{c}{ + 1.855 }\tabularnewline


==> border_tab/psnr_err2-tab-arri_ref.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 32.100 & 34.118 & 33.143 & 33.744 & 37.776 & 37.845 & 36.980 & 37.569 & 34.697 & 36.552\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.069 } & \multicolumn{2}{c}{ + 0.589 } & \multicolumn{2}{c}{ + 1.855 }\tabularnewline


==> border_tab/psnr_err2-tab-arri_ref_1row.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 32.100 & 34.118 & 33.143 & 33.744 & 37.776 & 37.845 & + 0.069 & 36.980 & 37.569 & + 0.589 & 34.697 & 36.552 & + 1.855\tabularnewline


==> border_tab/psnr_err2-tab-kodak.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 28.671 & 28.717 & 28.168 & 28.544 & 26.740 & 27.896\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.046 } & \multicolumn{2}{c}{ + 0.376 } & \multicolumn{2}{c}{ + 1.156 }\tabularnewline


==> border_tab/psnr_err2-tab-kodak_ref.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 24.975 & 26.215 & 25.998 & 26.073 & 28.671 & 28.717 & 28.168 & 28.544 & 26.740 & 27.896\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.046 } & \multicolumn{2}{c}{ + 0.376 } & \multicolumn{2}{c}{ + 1.156 }\tabularnewline


==> border_tab/psnr_err2-tab-kodak_ref_1row.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 24.975 & 26.215 & 25.998 & 26.073 & 28.671 & 28.717 & + 0.046 & 28.168 & 28.544 & + 0.376 & 26.740 & 27.896 & + 1.156\tabularnewline


==> border_tab/psnr_err2-tab-middleburry.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 39.998 & 40.061 & 39.238 & 39.789 & 37.038 & 38.805\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.063 } & \multicolumn{2}{c}{ + 0.551 } & \multicolumn{2}{c}{ + 1.767 }\tabularnewline


==> border_tab/psnr_err2-tab-middleburry_ref.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 34.048 & 36.429 & 35.529 & 35.821 & 39.998 & 40.061 & 39.238 & 39.789 & 37.038 & 38.805\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.063 } & \multicolumn{2}{c}{ + 0.551 } & \multicolumn{2}{c}{ + 1.767 }\tabularnewline


==> border_tab/psnr_err2-tab-middleburry_ref_1row.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 34.048 & 36.429 & 35.529 & 35.821 & 39.998 & 40.061 & + 0.063 & 39.238 & 39.789 & + 0.551 & 37.038 & 38.805 & + 1.767\tabularnewline


==> border_tab/psnr_err2-tab-tecnick.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 32.122 & 32.174 & 31.496 & 31.950 & 29.708 & 31.153\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.052 } & \multicolumn{2}{c}{ + 0.454 } & \multicolumn{2}{c}{ + 1.445 }\tabularnewline


==> border_tab/psnr_err2-tab-tecnick_ref.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 27.546 & 29.557 & 28.869 & 28.980 & 32.122 & 32.174 & 31.496 & 31.950 & 29.708 & 31.153\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.052 } & \multicolumn{2}{c}{ + 0.454 } & \multicolumn{2}{c}{ + 1.445 }\tabularnewline


==> border_tab/psnr_err2-tab-tecnick_ref_1row.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 27.546 & 29.557 & 28.869 & 28.980 & 32.122 & 32.174 & + 0.052 & 31.496 & 31.950 & + 0.454 & 29.708 & 31.153 & + 1.445\tabularnewline


==> tab/psnr-tab-arri.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 31.189 & 32.357 & 30.497 & 31.528 & 28.775 & 30.543\tabularnewline
 &  & \multicolumn{2}{c}{ + 1.168 } & \multicolumn{2}{c}{ + 1.031 } & \multicolumn{2}{c}{ + 1.768 }\tabularnewline


==> tab/psnr-tab-arri_ref.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 26.582 & 26.151 & 26.966 & 28.610 & 31.189 & 32.357 & 30.497 & 31.528 & 28.775 & 30.543\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 1.168 } & \multicolumn{2}{c}{ + 1.031 } & \multicolumn{2}{c}{ + 1.768 }\tabularnewline


==> tab/psnr-tab-kodak.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 25.419 & 25.764 & 24.998 & 25.447 & 23.895 & 24.856\tabularnewline
 & & \multicolumn{2}{c}{ + 0.345 } & \multicolumn{2}{c}{ + 0.449 } & \multicolumn{2}{c}{ + 0.961 }\tabularnewline


==> tab/psnr-tab-kodak_fres.tex <==
\multirow{2}{*}{\textit{Kodak}}  & NaN & NaN & NaN & NaN & NaN & NaN\tabularnewline


==> tab/psnr-tab-kodak_ref.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 21.952 & 21.476 & 23.264 & 23.856 & 25.419 & 25.764 & 24.998 & 25.447 & 23.895 & 24.856\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.345 } & \multicolumn{2}{c}{ + 0.449 } & \multicolumn{2}{c}{ + 0.961 }\tabularnewline


==> tab/psnr-tab-middleburry.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 34.912 & 35.025 & 34.225 & 34.481 & 33.086 & 33.874\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.113 } & \multicolumn{2}{c}{ + 0.256 } & \multicolumn{2}{c}{ + 0.788 }\tabularnewline


==> tab/psnr-tab-middleburry_ref.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 28.564 & 27.524 & 31.354 & 31.227 & 34.912 & 35.025 & 34.225 & 34.481 & 33.086 & 33.874\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.113 } & \multicolumn{2}{c}{ + 0.256 } & \multicolumn{2}{c}{ + 0.788 }\tabularnewline


==> tab/psnr-tab-tecnick.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 28.096 & 28.165 & 27.529 & 27.733 & 26.570 & 27.215\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.069 } & \multicolumn{2}{c}{ + 0.204 } & \multicolumn{2}{c}{ + 0.645 }\tabularnewline


==> tab/psnr-tab-tecnick_ref.tex <==
& \multirow{2}{*}{\textit{Tecnick}}  & 23.667 & 23.058 & 25.394 & 25.258 & 28.096 & 28.165 & 27.529 & 27.733 & 26.570 & 27.215\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.069 } & \multicolumn{2}{c}{ + 0.204 } & \multicolumn{2}{c}{ + 0.645 }\tabularnewline


==> tab/psnr_err2-tab-arri.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 34.875 & 37.648 & 33.919 & 37.206 & 29.815 & 35.936\tabularnewline
 &  & \multicolumn{2}{c}{ + 2.773 } & \multicolumn{2}{c}{ + 3.287 } & \multicolumn{2}{c}{ + 6.121 }\tabularnewline


==> tab/psnr_err2-tab-arri_ref.tex <==
 & \multirow{2}{*}{\textit{Arri}}  & 29.051 & 31.332 & 28.601 & 33.086 & 34.875 & 37.648 & 33.919 & 37.206 & 29.815 & 35.936\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 2.773 } & \multicolumn{2}{c}{ + 3.287 } & \multicolumn{2}{c}{ + 6.121 }\tabularnewline


==> tab/psnr_err2-tab-kodak.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 28.105 & 28.782 & 27.480 & 28.586 & 25.055 & 27.866\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.677 } & \multicolumn{2}{c}{ + 1.106 } & \multicolumn{2}{c}{ + 2.811 }\tabularnewline


==> tab/psnr_err2-tab-kodak_ref.tex <==
 & \multirow{2}{*}{\textit{Kodak}}  & 24.602 & 25.931 & 25.209 & 26.219 & 28.105 & 28.782 & 27.480 & 28.586 & 25.055 & 27.866\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.677 } & \multicolumn{2}{c}{ + 1.106 } & \multicolumn{2}{c}{ + 2.811 }\tabularnewline


==> tab/psnr_err2-tab-middleburry.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 39.545 & 39.913 & 38.777 & 39.634 & 36.305 & 38.667\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.368 } & \multicolumn{2}{c}{ + 0.857 } & \multicolumn{2}{c}{ + 2.362 }\tabularnewline


==> tab/psnr_err2-tab-middleburry_ref.tex <==
 & \multirow{2}{*}{\textit{Middleburry}}  & 33.979 & 36.285 & 35.359 & 35.278 & 39.545 & 39.913 & 38.777 & 39.634 & 36.305 & 38.667\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.368 } & \multicolumn{2}{c}{ + 0.857 } & \multicolumn{2}{c}{ + 2.362 }\tabularnewline


==> tab/psnr_err2-tab-tecnick.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 31.901 & 32.162 & 31.265 & 31.932 & 29.224 & 31.144\tabularnewline
 &  & \multicolumn{2}{c}{ + 0.261 } & \multicolumn{2}{c}{ + 0.667 } & \multicolumn{2}{c}{ + 1.920 }\tabularnewline


==> tab/psnr_err2-tab-tecnick_ref.tex <==
 & \multirow{2}{*}{\textit{Tecnick}}  & 27.618 & 29.552 & 28.851 & 28.674 & 31.901 & 32.162 & 31.265 & 31.932 & 29.224 & 31.144\tabularnewline
 &  & & & & & \multicolumn{2}{c}{ + 0.261 } & \multicolumn{2}{c}{ + 0.667 } & \multicolumn{2}{c}{ + 1.920 }\tabularnewline

